SSD: A Unified Framework for Self-Supervised Outlier Detection

We ask the following question: what training information is required to design an effective outlier/out-of-distribution (OOD) detector, i.e., detecting samples that lie far away from the training distribution? Since unlabeled data is easily accessible for many applications, the most compelling approach is to develop detectors based on only unlabeled in-distribution data. However, we observe that most existing detectors based on unlabeled data perform poorly, often equivalent to a random prediction. In contrast, existing state-of-the-art OOD detectors achieve impressive performance but require access to fine-grained data labels for supervised training. We propose SSD, an outlier detector based on only unlabeled in-distribution data. We use self-supervised representation learning followed by a Mahalanobis distance based detection in the feature space. We demonstrate that SSD outperforms most existing detectors based on unlabeled data by a large margin. Additionally, SSD even achieves performance on par, and sometimes even better, with supervised training based detectors. Finally, we expand our detection framework with two key extensions. First, we formulate few-shot OOD detection, in which the detector has access to only one to five samples from each class of the targeted OOD dataset. Second, we extend our framework to incorporate training data labels, if available. We find that our novel detection framework based on SSD displays enhanced performance with these extensions, and achieves state-of-the-art performance. Our code is publicly available at https://github.com/inspire-group/SSD.

==> Out of distribution detection with unlabeled data/def.tex <==
\newcommand{\dummytext}[1]{{\color{gray!25} #1}}
\definecolor{lightblue}{HTML}{507CB8}
\newcommand{\primaltext}[1]{{#1}}

\newcommand{\bluetext}[1]{{\color{black} #1}}
\newcolumntype{g}{>{\columncolor{gray!25}}c} % colored column

\newcommand{\ours}[1]{\textit{#1}}

% \ours{SSD\textsubscript{k}}

% \newcommand{\ssdksup}{$SSD_k$\raisebox{0.1em}{$+$}\xspace}
% \newcommand{\ssdsup}{$SSD$\raisebox{0.1em}{$+$}\xspace}
\newcommand{\ssdksup}{\ours{SSD\textsubscript{k}}\raisebox{0.1em}{$+$}\xspace}
\newcommand{\ssdsup}{\ours{SSD}\raisebox{0.1em}{$+$}\xspace}

\newcommand{\bcomment}[1]{}

\newcommand{\vikash}[1]{{\color{red} Vikash: #1}}
\newcommand{\algocomment}[1]{{\color{gray}\# #1}}


==> Out of distribution detection with unlabeled data/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\newcommand{\pin}{\hat{p}_{\rm{in}}}
\newcommand{\pood}{\hat{p}_{\rm{ood}}}


==> Out of distribution detection with unlabeled data/old_sections/intro.tex <==
Out-of-distribution detection aims to detect whether a particular input belongs to the training distribution. There are multiple approaches to solve this task in deep learning: using disciminative networks, Bayesian approaches, generative models. However, to the best of our understanding, discriminative approaches (Like ODIN, Mahalanobis detector), which are trained to solve a multi-class classification, achieves state-of-the-art detection performance. 


However, a key limitation of discriminate models is that they requirement fine-grained label information. Such information is crucial for them to develop an understanding of each class.\marginpar{\color{blue}\footnotesize first-motivation} However, labels are costly to obtain, and additionally acquiring fine-grained labels is even more costly (dog vs. breed of dog). In this work, \textit{we focus on OOD detection in a setting where no labels are present for in-distribution data}. 

OOD detection, without labels, is a similar setup as Outlier detection or anomaly detection. However, in deep learing, earlier approaches, such as Deep-SVDD~\cite{ruff18deepSvdd}, performs worse, even worse than generative models.\marginpar{\color{blue}\footnotesize first-goal} Our goal is to develop a method, which can compete, or even outperform, discriminative models while not requiring any labels. Note that to work well, both generative and Deep-SVDD model are further class-conditioned (since labels are available). We don't assume access to labels thus work without doing any class-conditioned modelling. 

Discriminative models leverage data labels achieve well clustered feature representations. Most detector leverage this property, with either using softmax scores or class conditional modeling of features representations. However, with increasing progress, self-supervised training methods are also able to improve feature representation, without needing any labels.\marginpar{\color{blue}\footnotesize first-observation} We argue that this ability of self-supervised methods can be distilled into a competitive OOD detector. 

Our approach is based on 1) segmenting self-supervised features in multiple clusters 2) measure entropy of each data points in each cluster 3) Using threshold on entropy to determine, if an input is OOD distribution. \marginpar{\color{blue}\footnotesize Summary-methods} Simply we base out detector on the observations that each clusters will be representative of a specific attribute of input data and OOD data might not be strongly represented by any of the clusters. We can name OOD detection based on such self-supervised approach as Self-Supervised Detection (\textbf{SSD}). 

This work can also be an opportunity to push for the following goals too:
\begin{itemize}
    \item \textit{How to validate detector performance on in-distribution data?} When claiming our detector have high TPR (validate all in-distribution images), we only test on the given training set. Should we be testing on a much larger rigorous set of images to claim that our detector does really have high TPR on the whole distribution, no just on the training set. Otherwise, the claims in the community are just getting overfitted to the images in our dataset, such as CIFAR10, which may not generalize to the whole distribution. Its similar to our ICCV idea of using transformations to expand in-distribution. 
    \item \textit{Using datasets representative of real-world setting?} What if we think of OOD detection from outlier/anomaly detection. Assuming that our only starting points is a set of inputs, where we don't even know which points are in or out distribution. We need to rethink the assumption that we always have a set of in-distribution images, as often we only have a set of in-distribution images, with OOD images present as label noise. Even more critical in learning without labels as the dataset are going to be even more uncontrolled.
    \item \textit{Asserting robust OOD detection.} In our earlier works we found that discriminative OOD detectors performs miserably when combined with robust training. \textbf{Would SSD better integrate with robust training}? But how do we craft an adversarial attacks and later design robust SSD.   
\end{itemize}

Note that our approach can also be integrated with supervised training, since supervised training achieves much better clustering in feature space, thus better detection performance than self-supervised features in out framework. 

\textbf{Assumptions.} Given the formulation of our approach, it will need calibration with some OOD data. We can provide results with two setting: 1) When no OOD data is available and we calibrate with random noise 2) When calibrating with OOD data. 


% Self-supervised learning is very effective in learning good clusters. However most methods operate under the assumption that fine-grained labels are available, thus supervised training. However, in real-world, OOD detection often translates to anomaly/outlier detection, where it may not be feasible to obtain labels in first place. Kind of like DeepSVM. Our question is how can be leverage the ability of these networks to do such amazing clustering to do better outlier detection. 

% We can then ask, how to develop robust self-supervised techniques focused on bringing robust clustering, thus better OOD detection performance in presence of adversary. Kind of giving more attention to our line of work. 

% I can also integrate it with my idea of using input transformation to help OOD detection.

==> Out of distribution detection with unlabeled data/old_sections/method.tex <==
Given a training set $\sX$ sample from $\pin$ consisting of training images $(\evx_1, \evx_2, \ldots, \evx_n)$, out objective to differentiate between $\sX$ and $\vz$, where $\vz \in \pood$. We first train a network with self-supervised method (SimCLR) to learn feature representations  $\sF = (\evf_1, \evf_2, \ldots, \evf_n)$. Our approach to develop a OOD detector on top of these representations takes the following steps:

\noindent \textbf{Step-1: Clustering.} In this step, we cluster the in-distribution features in $K$ clusters. Note that the choice of $K$ is pretty importance to success of out approach. We will use K-mean clustering in our work. It will return a set of centroids $\sC = (\evc_1, \evc_2, \ldots, \evc_k)$ for each clusters. Based on the distance to the cluster, the each point will be clustered with its nearest centroid, giving us a pseudo labels $\sY = (\evy_1, \evy_2, \ldots, \evy_n)$ for each training data point. 

\noindent \textbf{Step-2: Cluster-conditioned modelling of features vectors.} Our strategy is to develop a model of each cluster and use to detect OOD distribution data. The simplest model of all would be to use distance from cluster centroids. It includes, 1) Assign OOD features $\vf_z$ to the closest cluster $\evy_z$ 2) For each in-distribution data point in cluster $\evy_z$, find the distance from centroid, $S = \{d(\vf_i, \evc_{\evy_z}) | 1 \leq i \leq N, \evy_i = \evy_z\}$. Now $\vz$ will be OOD if $d(\vf_z, \evc_{\evy_z})\geq \delta$, where $\delta$ is determined from $\sS$ based on the pre-decided TPR (generally 95\%). 


\begin{figure}
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{temp/distance_low_entropy.png}
         \caption{Cluster where most examples are closest to the centroid (Tightest).}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{temp/distance_high_entropy.png}
         \caption{Cluster where most examples are farthest to the centroid (Loosest).}
     \end{subfigure}
    
    \caption{Two extremes of the clusters, tightest and loosest, obtained with Self-supervised training. Here we plot the distance distribution, for both in-distribution and OOD images belonging to each cluster. Again train data is used here as in-distribution.}
    \label{fig: distCluster}
\end{figure}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{temp/low_entropy_distribution.png}
         \caption{Cluster where most examples are closest to the centroid (Tightest).}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{temp/high_entropy_distribution.png}
         \caption{Cluster where most examples are farthest to the centroid (Loosest).}
     \end{subfigure}
    
    \caption{Simultaneously using distance from all clusters provide a better ability to differentiate between in and OOD data. Again train data is used here as in-distribution.}
\end{figure}


We show the results obtained with this approach in Figure~\ref{fig: distCluster}. It shows that distance from single cluster centroid will achieve poor OOD detection performance, since OOD data will be even closer to centroid in some clusters. 


We argue that dealing with each cluster individually is not the best strategy. We find that we should account distances from all clusters to better detect OOD data.\marginpar{\color{blue}\footnotesize Major-insight}. We first construct a vector $\vs$ where $\evs_{i} = -d(f, c_k)$ and $d$ is the $\normltwo$ distance. Our final score will be $H(\softmax(\vs))$, which is the entropy of the distribution obtained from distances from each cluster. We transform soft-max probabilities for simplicity. For better performance, we can also use distance like, Wasserstein, Mahalanobis distance to better compare with intra-cluster and inter-cluster data points. 


Hyper-parameters: Number of clusters (N), Temperature for softmax. 

==> Out of distribution detection with unlabeled data/old_sections/rel_work.tex <==
Note that we differ form the line of work which use self-supervision along with supervised training to improve OOD detectors~\cite{Winkens2020ContrastiveOOD, hendrycks2019SSLOOD}. We intend to use only Self-supervised learning, thus no labels, a setup which currently performs works in OOD detection. 

==> Out of distribution detection with unlabeled data/old_sections/results.tex <==
\begin{table}[!htb]
\centering
\caption{Comparison of our approach with state of the art detectors. Note that we are still using a sub-optimal setup (ResNet18 network, no hyperparameter tuning etc), as the goal was to get some quick numbers. Our method's performance is expected to improve further as we dig deeper. Note that all of these required labelled training data, and some even need OOD data for calibration, or pre-training on ImageNet. Our approach have none of these requirements and only require a set of unlabelled in-distribution images. We already achieve state-of-the-art FPR on CIFAR-10. Also CIFAR100 as OOD is hardest to detect, signalling that out methods performs best when the detection is hardest, a crucial innovation in OOD detection. We use features standardization following normalization, but removing former doesn't change much. Using best of distance or entropy$\times$distance, though entropy hurts with SVHN dataset and only helps barely when it does.}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{ccc|cc|cc}
\toprule
 & \multicolumn{2}{c}{CIFAR100} & \multicolumn{2}{c}{SVHN} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Gaussian \\ Noise\end{tabular}} \\  \cmidrule{2-3} \cmidrule{4-5} \cmidrule{6-7}
 & FPR (TPR=95)     & AUROC     & FPR (TPR=95)   & AUROC   & FPR (TPR=95)                              & AUROC  \\ \midrule
Softmax probability~\citep{hendrycks2016baseline} & -    & 86.4 & -   & 89.9 & -   & -     \\
ODIN~\cite{liang2017odin}          & -    & 85.8 & -   & 96.7 & -   & -     \\
Mahalanobis distance~\citep{lee2018unifiedOOD}    & -    & 88.2 & -   & 99.1 & -   & -     \\
Residual flows~\citep{zisselman2020resflow} & -    & 89.4 & -   & 99.1 & -   & -     \\
\textbf{Ours (100 clusters)}  & 57.1 & 87.5 & 13.0 & 97.6 & 2.4 & 98.9  \\
\textbf{Ours (500 clusters)}  & 57.3 & 87.9 & 12.1 & 97.8 & 2.3 & 98.7  \\
\textbf{Ours (2000 clusters)}  & \textbf{57.5} & \textbf{88.4} & \textbf{12.6} & \textbf{97.8} & 2.4 & 98.6  \\
%\textbf{Ours (10 clusters) + with labels}  & 64.6 & 84.3 & 46.3 & 91.8 & 3.1 & 99.1  \\
%\textbf{Ours (100 clusters) + with labels}  & 59.1 & 76.5 & 39.9 & 87.1 &  &   \\
%\textbf{Ours (500 clusters) + with labels}  & 58.3 & 77.2 & 38.6 & 88.3 &  &  \\  
Sup + Rotation-SSL~\citep{hendrycks2019SSLOOD} & -    & 90.9 & -   & 98.9 & -   & -     \\
Sup + SimCLR-SSL~\citep{Winkens2020ContrastiveOOD} (SOTA)  & \textbf{39.9} & \textbf{92.9} & \textbf{2.8} & \textbf{99.5} & 0.3 & 100.0 \\\bottomrule
\end{tabular}}
\end{table}


\begin{table}[!htb]
\centering
\caption{Using CIFAR100 as in-distribution, with ResNet18 network.}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{ccc|cc|cc}
\toprule
 & \multicolumn{2}{c}{CIFAR100} & \multicolumn{2}{c}{SVHN} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Gaussian \\ Noise\end{tabular}} \\  \cmidrule{2-3} \cmidrule{4-5} \cmidrule{6-7}
 & FPR (TPR=95)     & AUROC     & FPR (TPR=95)   & AUROC   & FPR (TPR=95)                              & AUROC  \\ \midrule
\textbf{Ours (100 clusters)}  & 73.4 & 78.8 & 26.9 & 91.7 & 4.4 & 98.7  \\
\textbf{Ours (500 clusters)}  & \textbf{68.6} & \textbf{80.8} & \textbf{20.2} & 93.1 & 3.0 & 98.8 \\
Sup + SimCLR-SSL~\citep{Winkens2020ContrastiveOOD} (SOTA)  &  81.8 & 78.3 & 23.3 & \textbf{95.6} & \textbf{0.2} & \textbf{99.9} \\ \bottomrule
\end{tabular}}
\end{table}


When labels are available, I find distance to closest cluster much better at OOD detection. With cifar10/cifar100 (in/ood) and 10 clusters combination it gets 46, 93.8 fpr and auroc respectively. With 100 clusters, we obtain 34 and 95.2 resectively. Increasingly number of clusters help but only with closest cluster distance, it hurts with entropy. \textit{If nothing else, just using cluster-conditional approach is sufficient to boost SOTA when labels are available.}


\subsection{Failure of statistical Outlier detection methods} Statistical methods for outlier detection assume that in-distribution data is generated from a certain distribution and OOD data will lie in its low-density regions. Generally, we assume that the distribution is Gaussian, where Mahalanobis distance can be used to characterize the equivalent high/low density regions. This works really well when we work with supervised training, since using Mahalanobis distance always works better than Euclidean, thus validating the assumption that Gaussian distribution is a nice prior. 

However, when working with OOD data (cifar10 as in-distribution) we observe that euclidean distance often works better than Mahalanobis, showing that Gaussian prior on data hurts more than it helps. Even more, performance with Mahalanobis distance gets even worse when we increase number of cluster, showing the individual clusters deviate even more from the Gaussian prior. Same behaviours occurs when we use a SupContrast model, i.e., model trained with both Supervised and Contrastive learning. Additionally, we find the SupContrast model, even with a single cluster, achieves SOTA on SVHN outlier dataset. This indicates that with labels, integrating them with Supervised learning might be more beneficial. 

\subsection{Beyond training dataset: validating TPR on training distribution}

As motivated earlier, it is imperative to validate the TPR of each detector on in-distribution images, going beyond the training set. With our detector, it is even more crucial, since a naive solution is assign each image a unique cluster. 
Don't forget to mention that performance on test can can certainly be used to check it.
\begin{table}[]
    \centering
    \caption{We select a select of 50k images from Tinyimages dataset which belongs to same class as CIFAR10, very likely in-distribution. When our detector is tuned to have TPR=95\% on CIFAR10 images, we test the TPR obtained in these tinyimages subset. Ideally, we would expect TPR=95\% on all indistribution images.}
    \begin{tabular}{ccc}
        \toprule
        Number of cluster &  TPR\\ \midrule
        100 &  87.9 \\
        500  & 82.3 \\
        2000 & 77.9 \\ \bottomrule
    \end{tabular}
\end{table}

List of our key observations is following:
\begin{itemize}
    \item We perform better in hard OOD setting than previous work. 
    \item Even with equal number of clusters, we beat previous SOTA on earlier datases. 
    \item 
\end{itemize}

==> Out of distribution detection with unlabeled data/sections/intro.tex <==
% \begin{wrapfigure}{r}{0.4\linewidth}
%  \vspace{-15pt}
%   \centering
%     \includegraphics[width=0.99\linewidth]{images/intro_simple.pdf}
%   \vspace{-10pt}
%   \caption{Detection performance with CIFAR-10 as in-distribution and CIFAR-100 as OOD dataset. SSD performs significantly better than existing detectors for unlabeled data and on par with supervised learning based detectors.}
%   \label{fig: intro}
%   \vspace{-10pt}
% \end{wrapfigure}

Deep neural networks are at the cornerstone of multiple safety-critical applications, ranging from autonomous driving~\citep{ramanagopal2018oodAV} to biometric authentication~\citep{masi2018deep, gunther2017opensetface}. When trained on a particular data distribution, referred to as in-distribution data, deep neural networks are known to fail against test inputs that lie far away from the training distribution, commonly referred to as outliers or out-of-distribution (OOD) samples~\citep{grubbs1969proceduresOOD, hendrycks2016baseline}. This vulnerability motivates the use of an outlier detector before feeding the input samples to the downstream neural network modules. 
%However, what information is \textit{crucial} to design an effective outlier detector? 
However, a key question is to understand what training information is \emph{crucial} for effective outlier detection? Will the detector require fine-grained annotation of training data labels or even access to a set of outliers in the training process?  

Since neither data labels nor outliers are ubiquitous, the most compelling option is to design outlier detectors based on only \emph{unlabeled} in-distribution data. However, we observe that most of the existing outlier detectors based on unlabeled data fail to scale up to complex data modalities, such as images. For example, autoencoder (AE)~\citep{hawkins2002outlierAE} based outlier detectors have achieved success in applications such as intrusion detection~\citep{mirsky2018kitsune}, and fraud detection~\citep{schreyer2017detection}. However, this approach achieves close to chance performance on image datasets. Similarly, density modeling based methods, such as PixelCNN++ \citep{salimans2017pixelcnn++} and Glow~\citep{kingma2018glow} are known to assign even a higher likelihood to outliers in comparison to in-distribution data~\citep{nalisnick2018dogenknow}.

In contrast, existing state-of-the-art OOD detectors achieve high success on image datasets but assume the availability of fine-grained labels for in-distribution samples~\citep{hendrycks2016baseline, cvpr16_open_set_networks, liang2017odin, dhamija2018agnostophobia, Winkens2020ContrastiveOOD}. This is a strong assumption since labels, in-particular fine-grained labels, can be very costly to collect in some applications~\citep{GoogleAIPricing2020}, which further motivates the use of unlabeled data. The inability of supervised detectors to use unlabeled data and poor performance of existing unsupervised approaches naturally give rise to the following question. 
%\vikash{Should we add the cifar-5,2 details which will require a forward reference to appendix from intro itself, won't look good.}



% \vikash{Should we give a forward reference to appendix from into itself? Or just avoid mentioning it.}

% What happens to the performance of current detectors if we relax this assumption with 1) assuming only coarse labels are present 2) only a small fraction of data is labeled. We simulate the first setup by combining consecutive class from CIFAR-10 dataset into two groups, referred to as CIFAR-2. For the second setup, we assume access to only 10\% of the training data. We use CIFAR-100 as the out-of-distribution dataset. Under both setups, we find the performance of existing detectors degrades significantly. These limitations of both supervised and unsupervised learning based detectors naturally give rise to the following question.

%Given the compelling motivation for using unlabeled training data and the poor performance of existing methods, the following question arises naturally. 

% The cost of label annotations, along with these limitations makes it compelling to develop outlier detectors with access to only unlabeled training data. 

\noindent\hspace{0.1\linewidth}\begin{minipage}{0.8\linewidth}
\textit{Can we design an effective {out-of-distribution (OOD) data detector} with access to only unlabeled data from training distribution?}
\end{minipage} 

A framework for outlier detection with unlabeled data\footnote{We refer to OOD detection without using class labels of in-distribution data as unsupervised OOD detection.} involves  two key steps: 1) Learning a good feature representation with unsupervised training methods 2) Modeling features of in-distribution data without requiring class labels. For example, autoencoders attempt to learn the representation with a bottleneck layer, under the expectation that successful reconstruction requires learning a good set of representations. Though useful for tasks such as dimensionality reduction, we find that these representations are not good enough to sufficiently distinguish in-distribution data and outliers. \primaltext{We argue that if unsupervised training can develop a rich understanding of key semantics in in-distribution data then absence of such semantics in outliers can cause them to lie far away in the feature space, thus making it easy to detect them}. Recently, self-supervised representation learning methods have made large progress, commonly measured by accuracy achieved on a downstream classification task~\citep{chen2020simclr, he2020moco, oord2018cpc, misra2020pirl, tian2020infomin}. We leverage these representations in our proposed cluster-conditioned framework based on the Mahalanobis distance~\citep{mahalanobis1936generalized}. Our key result is that self-supervised representations are highly effective for the task of outlier detection in our self-supervised outlier detection (\ours{SSD}) framework \primaltext{where they not only perform far better than most of the previous unsupervised representation learning methods but also perform on par, and sometimes even better, than supervised representations.} 

What if access to a fraction of OOD data or training data labels is available? How do we move past a detector based on unlabeled data and design a framework which can take advantage of such information? Though access to outliers during training is a strong assumption, it may be feasible to obtain a few prior instances of such outliers~\citep{gornitz2013toward}. We characterize this setting as \textit{few-shot OOD detection}, where we assume access to very few, often one to five, samples from the targeted set of outliers. While earlier approaches~\citep{liang2017odin, lee2018unifiedOOD} mostly use such data to calibrate the detector, we find that access to just a few outliers can bring an additional boost in the performance of our detector. Crucial to this success is the reliable estimation of first and second order statistics of OOD data in the high dimensional feature space with just a few samples. 
%\vikash{Should we give more details on how we did it.} We further extend our framework to take advantage of generic out-of-distribution samples.\vikash{Discuss earlier work on it} where we propose a novel modification of contrastive loss which optimize to make OOD samples equidistant from clusters of in-distribution data. 

%The success of self-supervised representation learning in SSD invokes the following questions. First, how uniquely suited are self-supervised representations for outlier detection compared to supervised methods? We aim to shed more light on it by comparing SSD with an equivalent supervised network in our results. Second, 

Finally, if class labels are available in the training phase, how can we incorporate them in the \ours{SSD} framework for outlier detection?  Recent works have proposed the addition of the supervised cross-entropy and self-supervised learning loss with a tunable parameter, which may require tuning for optimal parameter setting for each dataset~\citep{hendrycks2019rotnetOOD, Winkens2020ContrastiveOOD}. We demonstrate that incorporating labels directly in the contrastive loss achieves 1) a tuning parameter-free detector, and 2) \textit{state-of-the-art} performance.  

% Robust detection of outliers, i.e., samples which lie far away from training data distribution, at test time is crucial for safe deployment of deep neural networks in  critical applications. In designing outlier detection methods, a key question arises: what information about the training distribution is required for effective performance? 
% %
% %The key question is, what information is available for training distribution? 
% Does it suffice to have access to only unlabelled training data, since fine-grained labelling of data can be very costly?  
% %It is common to have access to only unlabelled training since fine-grained labelling of data can be very costly. 

% We find that existing outlier detection methods based on unlabelled data, such as methods based on reconstruction error from auto-encoders (cite) or density modelling (cite), perform poorly, often even worse than a randomly initialized neural network. On the other hand, while outlier detection methods based on supervised training on in-distribution data are able to achieve state-of-the-art success, they crucially rely on access to costly and fine-grained data labels. 
% %is critical to the success of state-of-the-art detectors, which leverage supervised training on in-distribution data.
% We demonstrate this in Figure xyz, where we combine classes of CIFAR-10 dataset to convert it from 10-class to a 5-class or 2-class classification dataset. We measure the success of the detector with Area under the ROC curve (AUROC), with higher AUROC indicating better performance. With the coarse labels, we observe consistent degradation in the performance of the detector. This poses the following challenge.

%------------------------------------------------------
% To solve this challenge, we propose \ours{SSD}, abbrv. for self-supervised detection, a outlier detection framework based on self-supervised representation learning on unlabelled data. We employ recently proposed contrastive self-supervised (cite) to learn a good feature representations. We then develop a cluster-conditioned detection framework, where we first clusters the features representations of training data and then model our detector based on Mahalnobis distance (cite) from individual clusters. We also thoroughly discuss the impact on distance metric and the number of clusters. 

% In some application, such a fraud detection, it might be feasible to develop a prior on the out-of-distribution (OOD) outliers. We characterize this setting as \textit{few-shot OOD detection}, where a assume access to very few, often one to five, samples from the targeted set of outliers. We extend our detector to this setting with following two novel methods: 1) Estimating covariance robustly a very few samples 2) Using data augmentation to increase the information in feature space. Even with one-shot, we find significant gain in performance with out approach. We also discuss its generalization to a novel set of outliers. 

% We further extend our framework to take advantage of generic out-of-distribution samples.\vikash{Discuss earlier work on it} We proposed a novel modification of contrastive loss where we also optimize to make OOD samples equidistant from clusters of in-distribution data. \vikash{Discuss its performance gains.} 

% Define and motivate the task of outlier/anomaly detection. Then argue that so many application require us to operated in a setup when no labels are available. Progress made but largely the most successful method require labels, but in learning feature representation for complex signal like images and further do a class-conditional modelling. Most earlier application are based on unsupervised representation learning methods like xyz. Not only they have low performance. But even when modelling class-wise, there performance remain far below supervised training methods. 
% \dummytext{\lipsum[66]}


% Overview on anomaly detection, outlier detection, ood detection, novelty detection. While having their subtle difference, argue how all requires fundamental ability to identify variation beyond the training distribution. Novelty/anomaly detection focus on subtle semantic variations (such as detecting novel species of birds when encountered for a bird-classification model), while outlier, ood detection also focus on more non-semantic variations.

% All of these applications have their independent applications. Novelty anomaly detection helps in making better decision (like bringing human in the loop) to get better utility. While outlier/ood detection can defend against unconstrained adversary by identifying even large degree of variations, which is often easier than novelty detection.

% Why this work is important when each domain is well studied. Though each domain is well-established, often that tools and techniques are simpler (for eg. using linear models, kernels as feature extractor). With complex modalities, such as vision, text, deep learning becomes a critical tool, and limited work exist on how to best harness its power to solves these challenges. We aim to bridge this gap in our work. 
% \dummytext{\lipsum[66]}


% We develop our experimental setup to reflect spirit of each of the four tasks: anomaly detection, outlier detection, novelty detection, ood detection. For examples, on ImageNet dataset, we test SSD with multiple set of anomalies ranging from small semantic variations to large deviations from in-distribution.
% \dummytext{\lipsum[66]}

\subsection{Key Contributions}
\noindent \textbf{\ours{SSD} for unlabeled data.} We propose \ours{SSD}, an unsupervised framework for outlier detection based on unlabeled in-distribution data. We demonstrate that \ours{SSD} outperforms most existing unsupervised outlier detectors by a large margin while also performing on par, and sometimes even better than supervised training based detection methods. We validate our observation across four different datasets: CIFAR-10, CIFAR-100, STL-10, and ImageNet. 

\noindent \textbf{Extensions of \ours{SSD}.} We provide two extensions of \ours{SSD} to further improve its performance. First, we formulate \textit{few-shot OOD detection} and propose detection methods which can achieve a significantly large gain in performance with access to only a few targeted OOD samples. Next, we extend \ours{SSD}, without using any tuning parameter, to also incorporate in-distribution data labels and achieve \textit{state-of-the-art} performance. 

==> Out of distribution detection with unlabeled data/sections/method.tex <==
In this section, we first provide the necessary background on outlier/out-of-distribution (OOD) detection and then present the underlying formulation of our self-supervised detector (\ours{SSD}) that relies on only unlabeled in-distribution data. Finally, we describe two extensions of \ours{SSD} to (optionally) incorporate targeted OOD samples and in-distribution data labels (if available). 

\noindent \textbf{Notation.} We represent the input space by $\mathcal{X}$ and corresponding label space as $\mathcal{Y}$. We assume in-distribution data is sampled from $\mathbb{P}_{\mathcal{X} \times \mathcal{Y}}^{in}$. In the absence of data labels, it is sampled from marginal distribution $\mathbb{P}_\mathcal{X}^{in}$. We sample out-of-distribution data from $\mathbb{P}_\mathcal{X}^{ood}$. We denote the feature extractor by $f: \mathcal{X} \to \mathcal{Z}$, where $\mathcal{Z} \subset \mathbb{R}^d$, a function which maps a sample from the input space to the $d$-dimensional feature space ($\mathcal{Z}$). The feature extractor is often parameterized by a deep neural network. In supervised learning, we obtain classification confidence for each class by $g \circ f : \mathcal{X} \to \mathbb{R}^c$. In most cases, $g$ is parameterized by a shallow neural network, generally a linear classifier. 

% For in-distribution data, we represent input space by $\mathcal{X}$ and each input sample as $x$. We represent its corresponding output label as $y$ and output space as $\mathcal{Y}$. We assume in-distribution data is sample from $\mathbb{P}_{X \times Y}^{in}$. In absence of data labels, it is samples from margin distribution $\mathbb{P}_X$. We represent an out-of-distribution sample as $z$, where $z \in \mathcal{Z}$, which is sampled from $\mathbb{P}_Z$. We denote the feature extractor by $f: \mathcal{X} \cup \mathcal{Z} \to \mathbb{R}^d$ a function which maps an point from the input space to a $d$-dimensional feature. The feature extractor is often parameterized by a deep neural network. In supervised learning, output confidence is achieved by $g \circ f : \mathcal{X} \to \mathbb{R}^c$. In most cases $g$ is parameterized by a shallow neural network, especially a linear classifier. 

%A range of successful works develop detection methods utilizing the information from features space and output confidence. However, common to their success is the use of in-distribution data labels, i.e., training the neural network ($f \circ g$) on $\mathbb{P}_{\mathcal{X} \times \mathcal{Y}}$ using supervised training techniques (CITE). Additionally the detection method also employ class labels to improve the performance. We refer this class of detector as \textit{supervised OOD detectors}. Even for generative, auto-encoders, and auto-regressive models, earlier work often use in-distribution data labels to do a class-conditional modelling, a key component in their success. \textit{Unsupervised OOD detectors} aim to solve the aforementioned OOD detection tasks, with access to only $\mathbb{P}_{\mathcal{X}}$.\vikash{Push some part in introduction, motivation. Also bring definition of unsupervised detectors here.}\vikash{Not just missing labels, but no semantic annotation is available (like hastags, bounding boxes), ref PIRL paper}

\noindent \textbf{Problem Formulation: Outlier/Out-of-distribution (OOD) detection.}  Given a collection of samples from $\mathbb{P}_\mathcal{X}^{in} \times \mathbb{P}_\mathcal{X}^{ood}$, the objective is to correctly identify the source distribution, i.e., $\mathbb{P}_\mathcal{X}^{in}$ or $\mathbb{P}_\mathcal{X}^{ood}$, for each sample. We use the term \textit{supervised OOD detectors} for detectors which use in-distribution data labels, i.e., train the neural network ($g \circ f$) on $\mathbb{P}_{\mathcal{X} \times \mathcal{Y}}^{in}$ using supervised training techniques. \textit{Unsupervised OOD detectors} aim to solve the aforementioned OOD detection tasks, with access to only $\mathbb{P}_{\mathcal{X}}^{in}$. In this work, we focus on developing effective unsupervised OOD detectors.

\noindent \textbf{Background: Contrastive self-supervised representation learning.} Given unlabeled training data, it aims to train a feature extractor, by discriminating between individual instances from data, to learn a good set of representations. 
Using image transformations, it first creates two views of each image, commonly referred to as positives. Next, it optimizes to pull each instance close to its positive instances while pushing away from other images, commonly referred to as negatives. Assuming that $(x_i, x_j)$ are positive pairs for the $i$th image from a batch of $N$ images and $h(.)$ is a projection header, $\tau$ is the temperature, contrastive training minimizes the following loss, referred to as Normalized temperature-scaled cross-entropy (\emph{NT-Xent}), over each batch.
\vspace{-5pt}
\begin{equation} \label{eq: simclr}
    \mathcal{L}_{batch}  = \frac{1}{2N}\sum_{i=1}^{2N}  -log\frac{e^{u_i^T u_j / \tau}}{\sum_{k=1}^{2N} \mathbbm{1}(k \neq i) e^{u_i^T u_k/\tau}}~~; ~~~~~~~~~ u_i = \frac{h\left(f(x_i)\right)}{\|h(f(x_i))\|_2}
    \vspace{-3pt}
\end{equation}

% where $h(.)$ is projection header which generally maps feature embeddings to a lower-dimensional space. To contrast with a large number of negatives, it requires a much larger batch size compared to the supervised cross-entropy loss function. 

% We would like to clarify that the notion of supervised detectors, refers to having access to labeled in-distribution data. It should not be confused with classical outlier detection literature, it is used to denote access to labeled outliers.

\subsection{Unsupervised outlier detection with SSD} 


\noindent \textbf{Leveraging contrastive self-supervised  training.} In the absence of data labels, \ours{SSD} consists of two steps: 1) Training a feature extractor using unsupervised representation learning, 2) Developing an effective OOD detector based on hidden features which isn't conditioned on data labels. 
\begin{wrapfigure}{r}{0.4\linewidth}
 \vspace{-10pt}
  \centering
  \includegraphics[width=\linewidth]{images/roc_vs_eigval.pdf}
  \vspace{-20pt}
  \caption{AUROC along individual principle eigenvector with CIFAR-10 as in-distribution and CIFAR-100 as OOD. Higher eigenvalues dominates euclidean distance, but are least helpful for outlier detection. Mahalnobis distance avoid this bias with appropriate scaling and performs much better.
  }
  \label{fig: why_mah}
  \vspace{-20pt}
\end{wrapfigure}
We leverage contrastive self-supervised training for representation learning in our outlier detection framework, particularly due to its state-of-the-art performance~\citep{chen2020simclr, tian2020infomin}. We will discuss the effect of different representation learning methods later in Section~\ref{subsec: ssdresults}.  



% Our objective with SSD is to achieve detection performance on par, or even better, with supervised detection methods. 

% it first requires learning a good set of features representation in an unsupervised manner and later developing effective detection methods which isn't conditioned on data labels. 

% Given a training set $\sX$ sample from $\pin$ consisting of training images $(\evx_1, \evx_2, \ldots, \evx_n)$, out objective to differentiate between $\sX$ and $\vz$, where $\vz \in \pood$. We first train a network with self-supervised method (SimCLR) to learn feature representations  $\sF = (\evf_1, \evf_2, \ldots, \evf_n)$. 
% \dummytext{\lipsum[5]} 

% Unsupervised representations learning can done using a wide-range of methods (list them). We argue that a crucial property of it for OOD detection is \emph{feature grouping}, i.e., ability to cluster semantically similar inputs together. Its can learn clusters at both coarse-level and fine-grained level (e.g., cluster for dog and cats or cluster for breeds of dogs). We aim to utilize this ability of unsupervised representation learning. Our hypothesis is that in absence of related semantic features, features for OOD data will be far away from clustered in-distribution data.



\noindent \textbf{Cluster-conditioned detection.} In absence of data labels, we develop a \textit{cluster-conditioned} detection method in the feature space. We first partition the features for in-distribution training data in \emph{m} clusters. We represent features for each cluster as $\mathcal{Z}_m$. We use k-means clustering method, due to its effectiveness and low computation cost. Next, we model features in each cluster independently, and calculate the following \textit{outlier score} ($s_x$) = $\displaystyle \min_{m}\mathcal{D}(x, \mathcal{Z}_m)$ for each test input $x$, where $\mathcal{D}(., .)$ is a distance metric in the feature space. %We use outlier scores of the test set of the in-distribution dataset and OOD dataset to discriminate between them. 
We discuss the choice of the number of clusters in Section~\ref{subsec: ssdresults}.

%\vikash{Describe a function for ood detection.}
%We discuss the effect of different clustering methods in Appendix xyz.

\noindent \textbf{Choice of distance metric: Mahalanobis distance.} We use  Mahalanobis distance to calculate the outlier score as follows: 
% \vspace{10pt}
\begin{equation}
    % \vspace{-10pt}
    s_x = \min_{m}(z_x - \mu_{m})^T \Sigma_m^{-1} (z_x - \mu_{m})
\end{equation}
where $\mu_m$ and $\Sigma_m$ are the sample mean and sample covariance of features ($\mathcal{Z}$) of the in-distribution training data. We justify this choice with quantitative results in Figure~\ref{fig: why_mah}. With eigendecomposition of sample covariance ($\Sigma_m = Q_m \Lambda_m Q_m^{-1}$), $\displaystyle s_x = \min_{m}\left(Q_m^T(z_x - \mu_{m})\right)^T \Lambda_m^{-1} \left (Q_m^T(z_x - \mu_{m})\right)$ which is equivalent to euclidean distance scaled with eigenvalues in the eigenspace. We discriminate between in-distribution (CIFAR-10) and OOD (CIFAR-100) data along each principal eigenvector (using AUROC, higher the better). With euclidean distance, i.e., in absence of scaling, components with higher eigenvalues have more weight but provide least discrimination. Scaling with eigenvalues removes the bias, making Mahalnobis distance effective for outlier detection in the feature space. 
%\primaltext{We provide a quantitative comparison between different distance metrics in Appendix~\ref{sec: appdistance}.}

% We experimented with multiple distance metrics, ranging from euclidean, cosine, Canberra, Chebyshev, and Mahalanobis distances


% \noindent \textbf{On choice of clustering.} While partitioning in-distribution data, number of clusters govern whether we model data at coarse-grained (small) or fine-grained (large) level. Note that even when unsupervised representation learning methods optimize at an instance level, since class labels are absent, it can learn a shared representation, capturing the salient semantics of in-distribution data. Our experimental results validates this hypothesis where non-trivial detection performance, even with modelling in-distribution representation of self-supervised methods as a single cluster. We also find the clustering can further helps to improve detection performance across both self-supervised and supervised methods. 

% Since covariance matrix is symmetric, and when its non-singular, it is diagonalizable, i.e, $\Sigma = Q \Lambda Q^{-1}$. Thus membership score is, 

% \begin{equation}
%     s_x = \min_{m}~\left(Q(x - \mu_{m})\right)^T \Delta_m^{-1} \left(Q^T(x - \mu_{m})\right)
% \end{equation}

% It is equivalent to first mapping the input to the eigen space and then scaling the euclidean distance with eigen value in each direction. Note that when 

 
% Discuss the choice of number of clusters. Do it only if the clusters are tight. Though current SSL learning methods might not be able to follow it. Show that clustering is a good idea and it helps terrifically, but kind of loses it value with self-supervised contrastive learning. See if we can provide an explanation for it. 


% \subsubsection{Experimental results for supporting analysis and design choices}
% Present some results in a minimal setting (rest in appendix). Kind of like "fast is better than free" paper. Just justify the design choice with step-by-step analysis.

% \textbf{SSD-ensembles.} We further proposed to boost the performance of SSD based on techniques to create an ensembles of multiple detectors.
% \begin{itemize}[noitemsep,topsep=0pt, leftmargin=15pt]
%     \item \noindent \textit{Ensembles based on sub-spaces.} We randomly select a fraction of dimension in feature vectors and calculate the membership score for each input. We aggregate the scores from different subspace in a additive manner. \vikash{Add a mathematical formulation.}
%     \item \noindent \textit{Ensembles based on sub-samples.} We randomly select a subset of training data to estimate the covariance and use it to calculate membership score for each test input. Again we aggregate the scores from multiple detectors by adding them. We didn't create ensembles based on different layers in the network. We find that features from earlier layers highly sub-optimal in OOD detection.
% \end{itemize}

% In the next few sections, we present the extension of our baseline detector in SSD framework.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Few-Shot OOD detection (\ours{SSD\textsubscript{k}})}
In this extension of the \ours{SSD} framework, we consider the scenario where a few samples from the OOD dataset {used at inference time} are also available at the time of training.
%It refers to OOD detection methods when a very small number of samples from the targeted distribution of anomalies are available when designing the method. 
We focus on \textit{one-shot} and \textit{five-shot} detection, which refers to access to only one and fives samples, from each class of the targeted OOD dataset, respectively. Our hypothesis is that in-distribution samples and OOD samples will be closer to other inputs from their respective distribution \emph{in the feature space}, while lying further away from each other. We incorporate this hypothesis by using following formulation of outlier score.
\begin{equation}
    \vspace{-5pt}
    s_x = (z_x - \mu_{in})^T \Sigma_{in}^{-1} (z_x - \mu_{in}) - (z_x - \mu_{ood})^T \Sigma_{ood}^{-1} (z_x - \mu_{ood})
\end{equation}

where $\mu_{in}, \Sigma_{in}$ and $\mu_{ood}, \Sigma_{ood}$ are the sample mean and sample covariance in the feature space for in-distribution and OOD data, respectively. 

\textbf{Challenge.} The key challenge is to reliably estimate the statistics for OOD data, with access to only a few samples. Sample covariance is not an accurate estimator of covariance when the number of samples is less than the dimension of feature space~\citep{stein1975coverror}, which is often in the order of thousands for deep neural networks.

\noindent \textbf{Shrunk covariance estimators and data augmentation.} We overcome this challenge by using following two techniques: 1) we use shrunk covariance estimators~\citep{ledoit2004shrunkcov}, and 2) we amplify number of OOD samples using data augmentation. We use shrunk covariance estimators due to their ability to estimate covariance better than sample covariance, especially when the number of samples is even less than the feature dimension. To further improve the estimation we amplify the number of samples using data augmentation at the input stage. We use common image transformations, such as geometric and photometric changes to create multiple different images from a single source image from the OOD dataset. Thus given a set of $k$ OOD samples $\{u_1, u_2, \ldots, u_k\}$, we first create a set of $k \times n$ samples using data augmentation, $\mathcal{U} = \{u_1^{1}, \ldots, u_1^{n}, \ldots u_k^{1}, \ldots, u_k^{n}\}$. Using this set, we calculate the outlier score for a test sample in the following manner.

\begin{equation} \label{eq : ssdk}
    \vspace{-5pt}
    s_x = (z_x - \mu_{in})^T \Sigma_{in}^{-1} (z_x - \mu_{in}) - (z_x - \mu_{U})^T S_{U}^{-1} (z_x - \mu_{U})
     \vspace{-5pt}
\end{equation}

where $\mu_{U}$ and $S_U$ are the sample mean and estimated covariance using shrunk covariance estimators for the set $\mathcal{U}$, respectively. 

% \vikash{Discuss the rate at which error in estimation of mean and samples decreases with samples. This will justify why we need way more samples to estimated covariance properly while not for mean}

% \noindent \textbf{Challenge:} Feature dimension in DNNs is 500-2000, thus it requires at least that many samples to estimate the full-rank covariance matrix. We show that an estimated covariance matrix can also be successfully used to improve the performance. Additional we use input data augmentation to increase the features in covariance estimation.
% \begin{equation*}
%     C_z = LWC(z_{T_1}, z_{T_2}, \ldots, z_{T_n})
% \end{equation*}
% where $LWC$ is Ledoit-Wolf covariance estimation and $z_{T_i}$ is the ith transformed version of an ood sample. Note that earlier works (like ODIN) have assumed access to ~1000 OOD samples. We are only assuming access to just a couple of them.
% \dummytext{\lipsum[11]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Integrating with generic OOD data.} How do we improve performance when we have access to generic OOD samples (similar to outlier exposure), e.g., Using tiny-images dataset as generic OOD dataset for cifar-10. With supervised training, we can maximize entropy, i.e., equal confidence for all classes. However, it's unclear what training objective to use for OOD data with self-supervised learning. We propose to optimize the following margin-based objective.
% \begin{equation}
%     L(.) = NT\text{-}Xent + \lambda * E\big[max(0, D(x, .) - D(z, .) + k)\big]
% \end{equation}
% where $D(x, .)$ corresponds to Mahalanobis distance of a given sample from the existing training samples. Minimizing the addition margin-based loss will force the network to networks to maximize distance for OOD data while minimizing it for in-distribution. However, to estimate mean and covariance, we need to extract features for all training data at every step. We show to using features from the last 10 batches suffice, which we store in the queue along with training. Thus the modified loss function comes at close to no computational overhead. With some early evaluation, we find that using the generic OOD dataset in SSL training indeed improves performance on multiple OOD datasets. For e.g., when detection cifar100 from cifar10, it improves the AUROC from 1-1.5\%. Since we finetune for a small number of epochs, we only end up using small fraction of ood data. Can we used with a pre-trained networks, even without access to original data. \vikash{Still setting on the final loss function. Will write it after that.}

\subsection{How to best use data labels (\ssdsup)} If fine-grained labels for in-distribution data are available, an immediate question is how to incorporate them in training to improve the success in detecting OOD samples. 

\noindent \textbf{Conventional approach: Additive self-supervised and supervised training loss.} A common theme in recent works (\citealt{hendrycks2019rotnetOOD, Winkens2020ContrastiveOOD}) is to
add self-supervised ($L_{ssl}$) and supervised ($L_{sup}$) training loss functions, i.e., $L_{training} = L_{sup} + \alpha L_{ssl}$, where the hyperparameter $\alpha$ is chosen for best performance on OOD detection. A common loss function for supervised training is cross-entropy.

\noindent \textbf{Our approach: Incorporating labels in contrastive self-supervised training.} As we show in Section~\ref{subsec: ssdresults}, even without labels, contrasting between instances using self-supervised learning is highly successful for outlier detection. 
%We find self-supervised contrastive training highly successful for OOD detection. Based on it, 
We argue for a similar instance-based contrastive training, where labels can also be incorporated to further improve the learned representations. To this end, we use the recently proposed supervised contrastive training loss function~\citep{khosla2020supcon}, which uses labels for a more effective selection of positive and negative instances for each image. In particular, we minimize the following loss function. 
\begin{equation}
    \mathcal{L}_{batch} = \frac{1}{2N}\sum_{i=1}^{2N}  -log\frac{ \frac{1}{2N_{y_i} - 1}\sum_{k=1}^{2N} \mathbbm{1}(k \neq i)\mathbbm{1}(y_k = y_i) e^{u_i^T u_k/\tau}}{\sum_{k=1}^{2N} \mathbbm{1}(k \neq i) e^{u_i^T u_k/\tau}}
\end{equation}

where $N_{y_i}$ refers to number of images with label $y_i$ in the batch. In comparison to contrastive NT-Xent loss (Equation~\ref{eq: simclr}), now we use images with  identical labels in each batch as positives. We will show the superior performance of this approach compared to earlier approaches, and note that it is also a parameter-free approach which doesn't require additional OOD data to tune parameters. \primaltext{We further use the proposed cluster-conditioned framework with Mahalnobis distance, as we find it results in better performance than using data labels.} We further summarize our framework in Algorithm~\ref{alg: ssd}.

\begin{minipage}[t]{0.99\textwidth}
\vspace{-10pt}
\begin{algorithm}[H]
% \vspace{-0.5cm}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwFunction{f}{getFeatures}
\SetKwFunction{fa}{SSDScore}
\SetKwFunction{fb}{SSDkScore}
\Input{$\mathcal{X}_{in}$, $\mathcal{X}_{test}$, feature extractor ($f$), projection head ($h$), Required True-positive rate ($T$), \textit{Optional}: $\mathcal{X}_{ood}, \mathcal{Y}_{in}$ \algocomment{$\mathcal{X}_{in} \in \mathbb{P}_{X}^{in}, \mathcal{X}_{ood} \in \mathbb{P}_{X}^{ood}$}} 
\Output{Is outlier or not? $\forall x \in \mathcal{X}_{test}$}
%\textbf{Function} features(\mathcal{X}: list) :
\textbf{Function }\emph{getFeatures($\mathcal{X}$): return }\{$f({x_i})/\|f({x_i})\|_2$, $\forall$ $x_i \in \mathcal{X}$\}\;
\textbf{Function }\emph{SSDScore($\mathcal{Z}, \mu, \Sigma$): return }\{$(z - \mu)^T \Sigma^{-1} (z - \mu)$, $\forall$ $z \in \mathcal{Z}$\}\;
\SetKwProg{Fna}{Function}{}{end}
\SetKwProg{Fnb}{Function}{}{end}
\Fna{SSDkScore($\mathcal{Z}, \mu_{in}, \Sigma_{in}, \mu_{ood}, \Sigma_{ood}$):}{return \{$(z - \mu_{in})^T \Sigma_{in}^{-1} (z - \mu_{in}) - (z - \mu_{ood})^T \Sigma_{ood}^{-1} (z - \mu_{ood})$, $\forall$ $z \in \mathcal{Z}$\ \};}
Parition $\mathcal{X}_{in}$ in training set ($\mathcal{X}_{train}$) and calibration set ($\mathcal{X}_{cal}$);\\
\uIf{$\mathcal{Y}_{in}$ is not available}
    {\scriptsize
    $\mathcal{L}_{batch} = \frac{1}{2N}\sum_{i=1}^{2N} -log\frac{e^{u_i^T u_j / \tau}}{\sum_{k=1}^{2N} \mathbbm{1}(k \neq i) e^{u_i^T u_k/\tau}}$; $u_i = \frac{h(f(x_i))}{\|h(f(x_i))\|_2};$ \algocomment{Train feature extractor}\\
    }
    \Else{
    \scriptsize
    $\mathcal{L}_{batch} = \frac{1}{2N} \sum_{i=1}^{2N}  -log\frac{\frac{1}{2N_{y_i} - 1}\sum_{k=1}^{2N} \mathbbm{1}(k \neq i)\mathbbm{1}(y_k = y_i) e^{u_i^T u_k/\tau}}{\sum_{k=1}^{2N} \mathbbm{1}(k \neq i) e^{u_i^T u_k/\tau}};$
    }
Train feature extractor ($f$) by minimizing $\mathcal{L}_{batch}$ over $\mathcal{X}_{train}$;\\
$\mathcal{Z}_{train} = \f(\mathcal{X}_{train})$, $\mathcal{Z}_{cal} = \f(\mathcal{X}_{cal})$\\
$\mathcal{Z}_{test} = \f(\mathcal{X}_{test})$, \textbf{if} $\mathcal{X}_{ood}$ \emph{is available}: $\mathcal{Z}_{ood} = \f(\mathcal{X}_{ood});$\\
\uIf{$\mathcal{X}_{ood}$ is not available}
    {
        $s_{cal} = \fa(\mathcal{Z}_{cal}, \mu_{train}, \Sigma_{train})$; \algocomment{Sample mean and convariance of $\mathcal{Z}_{train}$}\\
        $s_{test} = \fa(\mathcal{Z}_{test}, \mu_{train}, \Sigma_{train})$ \algocomment{outlier score};
    }
    \Else{
    \algocomment{Using convariance estimation techniques from Section 3.2 for $\mathcal{Z}_{ood}$}
    $s_{cal} = \fb(\mathcal{Z}_{cal}, \mu_{train}, \Sigma_{train}, \mu_{ood}, \Sigma_{ood})$; \\
        $s_{test} = \fb(\mathcal{Z}_{test}, \mu_{train}, \Sigma_{train}, \mu_{ood}, \Sigma_{ood})$;
    }
$x_i \in \mathcal{X}_{test}$ is an outlier if $s_{test}^i > (s_{cal}$ threshold at TPR = $T$);
\caption{Self-supervised outlier detection framework (\ours{SSD})}
\label{alg: ssd}
\end{algorithm}
\end{minipage}

% Question the additive approach used in earlier works~\cite{hendrycks2019SSLOOD, Winkens2020ContrastiveOOD}, i.e., adding supervised and self-supervised loss, and argue for supervised contrastive loss. We can do some simple theoretical analysis to see how gradients of supervised contrastive loss are better/different in appendix. \dummytext{\lipsum[11]}


==> Out of distribution detection with unlabeled data/sections/results.tex <==
\vspace{-5pt}
\subsection{Common setup across all experiments} \label{subsec: setup}
We use recently proposed NT-Xent loss function from SimCLR~\citep{chen2020simclr} method for self-supervised training. We use the ResNet-50 network in all key experiments but also provide ablation with ResNet-18, ResNet-34, and ResNet-101 network architecture. We train each network, for both supervised and self-supervised training, with stochastic gradient descent for 500 epochs, 0.5 starting learning rate with cosine decay, and weight decay and batch size set to 1e-4 and 512, respectively. We set the temperature parameter to 0.5 in the NT-Xent loss. We evaluate our detector with three performance metrics, namely FPR (at TPR=95\%), AUROC, and AUPR. For the supervised training baseline, we use identical training budget as \ours{SSD} while also using the Mahalanobis distance based detection in the feature space. Due to space constraints, we present results with AUROC, which refers to area under the receiver operating characteristic curve, in the main paper and provide detailed results with other performance metrics in Appendix~\ref{sec: appResultsMetric}. Our setup incorporates six image datasets along with additional synthetic datasets based on random noise. We report the average results over three independent runs in most experiments.

\noindent \textbf{Number of clusters.} We find the choice of the number of clusters dependent on which layer we extract the features from in the Residual neural networks. While for the first three blocks, we find an increase in AUROC with the number of clusters, the trend is reversed for the last block (Appendix~\ref{sec: appclusters}). Since the last block features achieve the highest detection performance, we model the in-distribution features as a single cluster in subsequent experiments.

% In absence of data labels, we use self-supervised representation learning to first train a feature extractor to learn general data representations. We later use these representations to calculate the membership score for each test input. Our key question is that in absence of data labels, how successful self-superivsed representation alone can be for OOD detection? 

% \textbf{Choice of unsupervised representation learning method and its relationship with clustering.} We experiment with xyz unsupervised representations learning methods and measure their success, with variation in number of clusters, in OOD detection. We present our results in Figure xyz. We find a \textit{positive correlation} (R value?) where better self-supervised representations i.e., achieves better accuracy on linear read-off, also achieve better results with OOD detection. SimCLR, a state-of-the-art self-supervised method based on contrastive training achieves highest performance. Our major findings is to uncover its performance with number of clusters, where unlike other methods, we find that increase in number of clusters degrades detection performance. We observe similar trend across varying datasets, SSD variations, and number of clusters (Appendix xyz). Based on this observation, we model representation learned by SimCLR as a single cluster in subsequent experiments. We report our experimental results in Table xyz and xyz, and provide an explict comparison below. Deep layer features fails to take advantage of clustering. On the other hand, with supervised representation, we find that performance improves with clustering. In Stl-10 we consider two setup. First low-data regime and second when even small amount of extra unlabeled data is used.

% Unsupervised outlier detection is notoriously hard. Earlier work on density-based models, shows that trained model on cifar-10 ends up assigning high probabilities to svhn (Nalisnick et al.). Ren et al. (likelihood ratio for OOD detection) improves it the AUROC to 93.3 still far below the 99.4 achieved by ODIN and others. Our work closes this gap by achieving 99.6 AUROC, even better than supervised methods. Even when VAE improves the reduces the reconstruction error of in-distribution, it fails to improve AUROC. Pitch rotnet as our effort in testing with other self-supervised techniques. 

\subsection{Performance of SSD} \label{subsec: ssdresults}
\noindent \textbf{Comparison with unsupervised learning based detectors.}
We present this comparison in Table~\ref{tab: comparison_unsup}. 
We find that \ours{SSD} improves average AUROC by up to 55, compared to standard outlier detectors based on Density modeling (PixelCNN++~\citep{salimans2017pixelcnn++}), input reconstruction (Auto-encoder~\citep{hawkins2002outlierAE}, Variational Auto-encoder~\citep{KingmaW13vae}), and One-class classification (Deep-SVDD~\cite{ruff18deepSvdd}). A common limitation of each of these three detectors is to find images from the SVHN dataset as more in-distribution when trained on CIFAR-10 or CIFAR-100 dataset. In contrast, \ours{SSD} is able to successfully detect a large fraction of outliers from SVHN dataset. We also experiment with Rotation-loss~\cite{gidaris2018rotnet}, a non-contrastive self-supervised training objective. We find that \ours{SSD} with contrastive NT-Xent loss achieves 9.6\% higher average AUROC compared to using Rotation-loss. 


\begin{table}[!t]
\centering
\vspace{-5pt}
\caption{Comparison of \ours{SSD} with different outlier detectors using only unlabeled training data.}
\vspace{-5pt}
\label{tab: comparison_unsup}
\begin{threeparttable}
\renewcommand{\arraystretch}{1.1}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
 \begin{tabular}[c]{@{}c@{}}\hspace{30pt}In-distribution\\  \hspace{30pt}(Out-of-distribution)\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}CIFAR-10\\  (SVHN)\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}CIFAR-10 \\ (CIFAR-100)\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}CIFAR-100\\ (SVHN)\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}CIFAR-100\\ (CIFAR-10)\end{tabular} &  & Average \\ \midrule
 Autoencoder~\citep{hawkins2002outlierAE} &  & 2.5 &  & 51.3 &  & 3.0 &  & 51.4 &  & 27.0 \\
 VAE \citep{KingmaW13vae} &  & 2.4 &  & 52.8 &  & 2.6 &  & 47.1 &  & 26.2 \\
 PixelCNN++ \citep{salimans2017pixelcnn++} &  & 15.8 &  & 52.4 &  & -- &  & -- &  & -- \\
 Deep-SVDD \citep{ruff18deepSvdd} &  & 14.5 &  & 52.1 &  & 16.3 &  & 51.4 &  & 33.5 \\
 Rotation-loss~\citep{gidaris2018rotnet} &  & 97.9 &  & 81.2 &  & 94.4 &  & 50.1 &  & 80.9 \\
   {CSI \citep{tack2020csi}} &  & \textbf{99.8} &  & 89.2 &  & -- &  & -- &  & -- \\
\ours{SSD} &  & 99.6 &  & \textbf{90.6} &  & \textbf{94.9} &  & \textbf{69.6} &  & \textbf{88.7} \\
\ours{SSD\textsubscript{k}} ($k$ = 5) &  & \textbf{99.7} &  & \textbf{93.1} &  & \textbf{99.1} &  & \textbf{78.2} &  & \textbf{92.5} \\ \bottomrule
\end{tabular}
}
\end{threeparttable}
\vspace{-10pt}
\end{table}

\noindent \textbf{Ablation studies.}
We ablate along individual parameters in self-supervised training with CIFAR-10 as in-distribution data (Figure~\ref{fig: ablation}). While architecture doesn't have a very large effect on AUROC for most OOD dataset, we find that the number of training epochs and batch size plays a key role in detecting outliers from the CIFAR-100 dataset, which is hardest to detect among the four OOD datasets. We also find an increase in the size of training dataset helpful in the detection of all four OOD datasets.

\begin{figure}[!htb]
    \vspace{-5pt}
    \centering
    \begin{subfigure}[b]{0.24\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{images/roc_vs_arch.pdf}
        \caption{Model size.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{images/roc_vs_epochs.pdf}
        \caption{Number of epochs.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{images/roc_vs_batchsize.pdf}
        \caption{Batch size.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{images/roc_vs_samples.pdf}
        \caption{Size of training set.}
    \end{subfigure}
    \vspace{-5pt}
    \caption{Ablating across different training parameters in \ours{SSD} under following setup: In-distribution dataset = CIFAR-10, OOD dataset = CIFAR-100, Training epochs = 500, Batch size = 512.}
    \label{fig: ablation}
    \vspace{-5pt}
\end{figure}

\noindent \textbf{Comparison with supervised representations.}  We earlier asked the question \textit{ whether data labels are even necessary to learn representations crucial for OOD detection?} To answer it, we compare \ours{SSD} with a supervised network, trained with an identical budget as \ours{SSD} while also using Mahalanobis distance in the feature space, across sixteen different pairs of in-distribution and out-of-distribution datasets (Table~\ref{tab: allresults}). We observe that self-supervised representations even achieve better performance than supervised representations for 56\% of the tasks in Table~\ref{tab: allresults}. 

{
\noindent \textbf{Success in anomaly detection}. We now measure the performance of \ours{SSD} in anomaly detection where we consider one of the CIFAR-10 classes as in-distribution and the rest of the classes as a source of anomalies. Similar to the earlier setup, we train a ResNet-50 network using self-supervised training with NT-Xent loss function. While the contrastive loss attempt to separate individual instances in the feature space, we find that adding an $\ell_2$ regularization in the feature space helps in improving performance. In particular, we add this regularization (with a scaling coefficient of 0.01) to bring individual instance features close to the mean of all feature vectors in the batch. Additionally, we reduce the temperature from 0.5 to 0.1 to reduce the separability of individual instances due to the contrastive loss. Overall, we find that our approach outperforms all previous works and achieves competitive performance with the concurrent work of \cite{tack2020csi} (Table~\ref{tab: anodet}).
}

% \noindent \textbf{Integration with generic OOD data.} Similar to~\cite{hendrycks2018OE}, we use CIFAR-10 as in-distribution dataset and the 80M Tiny-Images dataset, after removing CIFAR-10 images from it, as the source of a generic OOD dataset. \vikash{Discuss results}. Note that we don't include the generic OOD data in other experiments of our paper. \vikash{Make sure to discuss the effect of number of clusters.}

\begin{table}[!htb]
\caption{Comparing performance of self-supervised (\ours{SSD}) and supervised representations. We also provide results for few-shot OOD detection (\ours{SSD\textsubscript{k}}) for comparison with our baseline \ours{SSD} detector.}
\vspace{-5pt}
\label{tab: allresults}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{cccc|cccccccc|cc}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}In-\\ distribution\end{tabular}} & \multirow{2}{*}{OOD} & \multirow{2}{*}{\ours{SSD}} & \multirow{2}{*}{Supervised} & \multicolumn{2}{c}{\ours{SSD\textsubscript{k}}} &  &  &  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}In-\\ distribution\end{tabular}} & \multirow{2}{*}{OOD} & \multirow{2}{*}{\ours{SSD}} & \multirow{2}{*}{Superivsed} & \multicolumn{2}{c}{\ours{SSD\textsubscript{k}}} \\ 
 &  &  &  & k=1 & k=5 &  &  &  &  &  &  &  k=1 & k=5 \\ \cmidrule{1-6} \cmidrule{8-14}
\multirow{5}{*}{CIFAR-10} & CIFAR-100 & 90.6 & 90.6 & 91.7 & 93.0 &  &   & \multirow{4}{*}{STL-10} & CIFAR-100 & \textbf{94.8} & 84.0 & 90.1 & 90.0 \\  
 & SVHN & 99.6 & 99.6 & 99.9 & 99.7 &  &  &  & SVHN & \textbf{98.7} & 95.7 & 98.7 & 99.4 \\  
 & Texture & 97.6 & \textbf{97.8} & 98.9 & 99.4 &  &  &  & Texture & \textbf{85.8} & 75.5 & 85.7 & 84.5 \\   
 & Blobs & 98.8 & \textbf{99.9} & 99.7 & 100.0 &  &  &  & Blobs & \textbf{96.4} & 88.6 & 96.5 & 99.9 \\  
& {LSUN} & \textbf{96.5} & 93.8 & 97.6 & 97.8 &  &  &  & {LSUN} & \textbf{88.8} & 66.8 & 94.1 & 94.5 \\  
& {Places365} & \textbf{95.2} & 92.7 & 96.7 & 97.3 &  &  &  & {Places365} & \textbf{88.3} & 64.9 & 95.4 & 95.6 \\  \cmidrule{1-6} \cmidrule{8-14}
\multirow{4}{*}{CIFAR-100} & CIFAR-10 & \textbf{69.6} & 55.3 & 74.8 & 78.3 &  &  &  \multirow{4}{*}{ImageNet} & SVHN & 99.1 & \textbf{99.4} & 99.7 & 100.0 \\    
 & SVHN & \textbf{94.9} & 94.5 & 99.5 & 99.1 &  &  &  & Texture & \textbf{95.4} & 85.1 & 94.7 & 97.3 \\  
 & Texture & 82.9 & \textbf{98.8} & 96.8 & 94.2 &  &  &  & Blobs & \textbf{99.5} & 98.4 & 100.0 & 100.0 \\  
 & Blobs & \textbf{98.1} & 57.3 & 98.1 & 100.0 &  &  &   &  Gaussian Noise & 100.0 & 100.0 & 100.0 & 100.0 \\  
 & { LSUN} & \textbf{79.5} & 69.4 & 92.3 & 93.4 &  &  &  & {ImageNet-O} & 45.2 & \textbf{75.5} & 89.4 & 93.3 \\  
 & {Places365} & \textbf{79.6} & 62.6 & 90.7 & 92.7 &  &  &  &  &  &  &  &  \\  \bottomrule
\end{tabular}}
\vspace{-5pt}
\end{table}

% \noindent \textbf{Success with ensembles.} Discuss that assembling can further improves the performance. However, to avoid overcrowding the methods, we choose not to use ensembling in other reported experimental results. Note that ensembles are used a inference stage and doesn't require modifying the training part of detector. 



\begin{table}[!htb]
\centering
\footnotesize
\caption{Comparison of \ours{SSD} with other detectors for anomaly detection task on CIFAR-10 dataset.}
\vspace{-5pt}
\label{tab: anodet}
\renewcommand{\arraystretch}{1.1}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{cccccccccccc} 
\toprule
 & Airplane & Automobile & Bird & Cat & Deer & Dog & Frog & Horse & Ship & Truck & Average \\ \midrule
Randomly Initialized network & 77.4 & 44.1 & 62.4 & 44.1 & 62.1 & 49.6 & 59.8 & 48.0 & 73.8 & 53.7 & 57.5 \\
VAE~\citep{KingmaW13vae} & 70.0 & 38.6 & 67.9 & 53.5 & 74.8 & 52.3 & 68.7 & 49.3 & 69.6 & 38.6 & 58.3 \\
OCSVM~\citep{scholkopf2001ocsvm} & 63.0 & 44.0 & 64.9 & 48.7 & 73.5 & 50.0 & 72.5 & 53.3 & 64.9 & 50.8 & 58.5 \\
AnoGAN~\citep{schlegl2017anogan} & 67.1 & 54.7 & 52.9 & 54.5 & 65.1 & 60.3 & 58.5 & 62.5 & 75.8 & 66.5 & 61.8 \\
PixelCNN~\citep{van2016pixcnn} & 53.1 & 99.5 & 47.6 & 51.7 & 73.9 & 54.2 & 59.2 & 78.9 & 34.0 & 66.2 & 61.8 \\
DSVDD~\citep{ruff18deepSvdd} & 61.7 & 65.9 & 50.8 & 59.1 & 60.9 & 65.7 & 67.7 & 67.3 & 75.9 & 73.1 & 64.8 \\
OCGAN~\citep{perera2019ocgan} & 75.7 & 53.1 & 64.0 & 62.0 & 72.3 & 62.0 & 72.3 & 57.5 & 82.0 & 55.4 & 65.6 \\
RCAE~\citep{chalapathy2018rcae} & 72.0 & 63.1 & 71.7 & 60.6 & 72.8 & 64.0 & 64.9 & 63.6 & 74.7 & 74.5 & 68.2 \\
DROCC~\citep{goyal2020DROCC} & 81.7 & 76.7 & 66.7 & 67.1 & 73.6 & 74.4 & 74.4 & 71.4 & 80.0 & 76.2 & 74.2 \\
Deep-SAD~\citep{ruff2019deepSAD} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & 77.9 \\
E3Outlier~\citep{wang2019E3Outlier} & 79.4 & 95.3 & 75.4 & 73.9 & 84.1 & 87.9 & 85.0 & 93.4 & 92.3 & 89.7 & 85.6 \\
GT~\citep{golan2018GT} & 74.7 & 95.7 & 78.1 & 72.4 & 87.8 & 87.8 & 83.4 & 95.5 & 93.3 & 91.3 & 86.0 \\
InvAE~\citep{huang2019InvAE} & 78.5 & 89.8 & 86.1 & 77.4 & 90.5 & 84.5 & 89.2 & 92.9 & 92.0 & 85.5 & 86.6 \\
GOAD~\citep{Bergman2020GOAD} & 77.2 & 96.7 & 83.3 & 77.7 & 87.8 & 87.8 & 90.0 & 96.1 & 93.8 & 92.0 & 88.2 \\
CSI~\citep{tack2020csi} & 89.9 & 99.9 & 93.1 & 86.4 & 93.9 & 93.2 & 95.1 & 98.7 & 97.9 & 95.5 & 94.3 \\ 
\ours{SSD} & 82.7 & 98.5 & 84.2 & 84.5 & 84.8 & 90.9 & 91.7 & 95.2 & 92.9 & 94.4 & 90.0 \\ \bottomrule
\end{tabular}}
\vspace{-10pt}
\end{table}




\subsection{Few-shot OOD detection (\ours{SSD\textsubscript{k}})} \label{subsec: ssdkresults}
\noindent \textbf{Setup.} We focus on one-shot and five-shot OOD detection, i.e., set $k$ to 1 or 5 in Equation~\ref{eq : ssdk} and use Ledoit-Wolf~\citep{ledoit2004shrunkcov} estimator for covariance estimation. To avoid a bias on selected samples, we report average results over 25 random trials.

%With CIFAR10 as the OOD dataset, it means access to one and five images, respectively, from each class. We create 10 randomly transformed samples from each available OOD image. To avoid any hyperparameter selection, we use the image augmentation technique to be the same as the one used in training. Finally, we use Ledoit-Wolf~\citep{ledoit2004shrunkcov} estimator to estimate the covariance.  \vikash{ToDo.}

\noindent \textbf{Results.} Compared to the baseline \ours{SSD} detector, one-shot and five-shot settings improve the average AUROC, across all OOD datasets, by 1.6 and 2.1, respectively (Table~\ref{tab: comparison_unsup}, \ref{tab: allresults}). In particular, we observe large gains with CIFAR-100 as in-distribution and CIFAR-10 as OOD where five-shot detection improves the AUROC from 69.6 to 78.3. We find the use of shrunk covariance estimator most critical in the success of our approach. Use of shrunk covariance estimation itself improves the AUROC from 69.6 to 77.1. Then data augmentation further improves it 78.3 for the five-shot detection. With an increasing number of transformed copies of each sample, we also observe improvement in AUROC, though it later plateaus close to ten copies (Appendix~\ref{sec: appfewshot}).

\noindent \textbf{What if additional OOD images are available} Note that some earlier works, such as \cite{liang2017odin}, assume that 1000 OOD inputs are available for tuning the detector. We find that with access to this large amount of OOD samples, \ours{SSD\textsubscript{k}} can improve the state-of-the-art by an even larger margin. For example, with CIFAR-100 as in-distribution and CIFAR-10 as out-of-distribution, it achieves 89.4 AUROC, which is 14.2\% higher than the current state-of-the-art~\citep{Winkens2020ContrastiveOOD}. 
%To put this improvement in context, this is the \textit{single largest} gain as the over last few year, AUROC has only improved from 77.1~\citep{hendrycks2016baseline} to 78.3~\citep{Winkens2020ContrastiveOOD}.  We provide additional results with access to varying number of OOD images in Appendix xyz. 

\subsection{Success when using data labels (\ssdsup)} \label{subsec: ssdsupesults}
Now we integrate labels of training data in our framework and compare it with the existing state-of-the-art detectors. We report our results in Table~\ref{tab: supresults}. Our approach improves the average AUROC by 0.8 over the previous state-of-the-art detector. Our approach also achieves equal or better performance than previous state-of-the-art across individual pairs of in and out-distribution dataset. For example, using labels in our framework improves the AUROC of Mahalanobis detector from 55.5 to 72.1 for CIFAR-100 as in-distribution and CIFAR-10 as the OOD dataset. Using the simple softmax probabilities,  training a two-layer MLP on learned representations further improves the AUROC to 78.3. Combining \ssdsup with a five-shot OOD detection method further brings a gain of 1.4 in the average AUROC.

\begin{table}[!htb]
\centering
\footnotesize
\caption{Comparison of \ssdsup, i.e., incorporating labels in the \ours{SSD} detector, with state-of-the-art detectors based on supervised training.}
\label{tab: supresults}
\vspace{-5pt}
\begin{threeparttable}
\renewcommand{\arraystretch}{1.1}
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
 \begin{tabular}[c]{@{}c@{}}\hspace{50pt}In-distribution\\  \hspace{50pt}(Out-of-distribution)\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}CIFAR-10\\  (CIFAR-100)\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}CIFAR-10 \\ (SVHN)\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}CIFAR-100\\ (CIFAR-10)\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}CIFAR-100\\ (SVHN)\end{tabular} &  & Average \\ \midrule
 Softmax-probs~\citep{hendrycks2016baseline} &  & 89.8 &  & 95.9 &  & 78.0 &  & 78.9 &  & 85.6 \\
 ODIN\tnote~\citep{liang2017odin}{$\dagger$} &  &  89.6 &  & 96.4 &  & 77.9 &  & 60.9 &  &  81.2 \\
 Mahalnobis~\citep{lee2018unifiedOOD}\tnote{$\dagger$} &  & 90.5 &  & 99.4 &  & 55.3 &  & 94.5 &  & 84.8 \\
 Residual Flows~\citep{zisselman2020resflow}\tnote{$\dagger$} &  & 89.4 &  & 99.1 &  & 77.1 &  & \textbf{97.5} &  & 90.7 \\
 Gram Matrix~\citep{sastry2019detecting} &  & 79.0 &  & 99.5 &  & 67.9 &  & 96.0 &  & 85.6 \\
 Outlier exposure \citep{hendrycks2018OE} &  & 93.3 &  & 98.4 &  & 75.7 &  & 86.9 &  & 88.6 \\
 Rotation-loss + Supervised \citep{hendrycks2019rotnetOOD} &  & 90.9 &  & 98.9 &  & -- &  & -- &  & -- \\
 Contrastive + Supervised \citep{Winkens2020ContrastiveOOD}\tnote{*} &  & 92.9 &  & 99.5 &  & \textbf{78.3} &  & 95.6 &  & 91.6 \\ 
 {CSI \citep{tack2020csi}} &  & 92.2 &  & 97.9 &  & -- &  & -- &  & -- \\ \cmidrule{1-11}
 \ssdsup &  & \textbf{93.4} &  & \textbf{99.9} &  & \textbf{78.3} &  & \textbf{98.2} &  & \textbf{92.4} \\
 \ssdksup ($k$ = 5)  &  & \textbf{94.1} &  & \textbf{99.6} &  & \textbf{84.1} &  & \textbf{97.4} &  & \textbf{93.8} \\ \bottomrule
\end{tabular}}
\begin{tablenotes}
{\scriptsize \item[] $^*$ Uses 4$\times$ wider ResNet-50 network, $^\dagger$ Requires additional out-of-distribution data for tuning.}
\vspace{-15pt}
\end{tablenotes}
\end{threeparttable}
\end{table}




% \begin{table}[!htb]
% \centering
% \footnotesize
% \caption{Comparison of \ssdsup, i.e., incorporating labels in the $SSD$ detector, with state-of-the-art detectors based on supervised training.}
% \label{tab: supresults}
% \vspace{-5pt}
% \begin{threeparttable}
% \renewcommand{\arraystretch}{1.1}
% \resizebox{0.5\linewidth}{!}{
% \begin{tabular}{lcc}
% \toprule
%  \begin{tabular}[c]{@{}c@{}}\hspace{50pt}In-distribution\\  \hspace{50pt}(Out-of-distribution)\end{tabular} &  & Average \\ \midrule
%  Softmax-probs~\citep{hendrycks2016baseline} &  & 85.6 \\
%  ODIN\tnote~\citep{liang2017odin}{$\dagger$} &  &  81.2 \\
%  Mahalnobis~\citep{lee2018unifiedOOD}\tnote{$\dagger$} &  & 84.8 \\
%  Residual Flows~\citep{zisselman2020resflow}\tnote{$\dagger$} &  & 90.7 \\
%  Gram Matrix~\citep{sastry2019detecting} &  & 85.6 \\
%  Outlier exposure \citep{hendrycks2018OE} &  & 88.6 \\
%  Contrastive + Supervised \citep{Winkens2020ContrastiveOOD}\tnote{*} &  & 91.6 \\ 
%  \cmidrule{1-3}
%  \ssdsup &  & \textbf{92.4} \\
%  \ssdksup ($k$ = 5)  &  & \textbf{93.8} \\ \bottomrule
% \end{tabular}}
% \begin{tablenotes}
% {\scriptsize \item[] $^*$ Uses 4$\times$ wider ResNet-50 network, $^\dagger$ Requires additional out-of-distribution data for tuning.}
% \vspace{-15pt}
% \end{tablenotes}
% \end{threeparttable}
% \end{table}




==> Out of distribution detection with unlabeled data/sections/setup.tex <==





% \noindent \textbf{Architectures.} Given the large batch requirement of SimCLR, we use a ResNet50 network. Unlike previous works we don't use a highly over-parameterized wrn-28-10. 

% \noindent \textbf{Metrics.} Mention only a few and push the rest, both their definition and results, in appendix.

% \noindent \textbf{Datasets.} For each dataset mention which data points we consider as OOD and which as in-distribution.

% \subsubsection{Evaluation protocols}
% \noindent \textbf{Dataset based.} Here we use another dataset as OOD. Easiest to detect.

% \noindent \textbf{Class/Semantics based.} Here we use another dataset as OOD.

\noindent \textbf{Baselines.} We compare with earlier work on unsupervised modelling of in-distribution data. In particular, we use auto-encoders and autoregressive models as the baseline. We also compare with an equivalent supervised network along with with  existing state of the art.






==> old_sections/intro.tex <==
Out-of-distribution detection aims to detect whether a particular input belongs to the training distribution. There are multiple approaches to solve this task in deep learning: using disciminative networks, Bayesian approaches, generative models. However, to the best of our understanding, discriminative approaches (Like ODIN, Mahalanobis detector), which are trained to solve a multi-class classification, achieves state-of-the-art detection performance. 


However, a key limitation of discriminate models is that they requirement fine-grained label information. Such information is crucial for them to develop an understanding of each class.\marginpar{\color{blue}\footnotesize first-motivation} However, labels are costly to obtain, and additionally acquiring fine-grained labels is even more costly (dog vs. breed of dog). In this work, \textit{we focus on OOD detection in a setting where no labels are present for in-distribution data}. 

OOD detection, without labels, is a similar setup as Outlier detection or anomaly detection. However, in deep learing, earlier approaches, such as Deep-SVDD~\cite{ruff18deepSvdd}, performs worse, even worse than generative models.\marginpar{\color{blue}\footnotesize first-goal} Our goal is to develop a method, which can compete, or even outperform, discriminative models while not requiring any labels. Note that to work well, both generative and Deep-SVDD model are further class-conditioned (since labels are available). We don't assume access to labels thus work without doing any class-conditioned modelling. 

Discriminative models leverage data labels achieve well clustered feature representations. Most detector leverage this property, with either using softmax scores or class conditional modeling of features representations. However, with increasing progress, self-supervised training methods are also able to improve feature representation, without needing any labels.\marginpar{\color{blue}\footnotesize first-observation} We argue that this ability of self-supervised methods can be distilled into a competitive OOD detector. 

Our approach is based on 1) segmenting self-supervised features in multiple clusters 2) measure entropy of each data points in each cluster 3) Using threshold on entropy to determine, if an input is OOD distribution. \marginpar{\color{blue}\footnotesize Summary-methods} Simply we base out detector on the observations that each clusters will be representative of a specific attribute of input data and OOD data might not be strongly represented by any of the clusters. We can name OOD detection based on such self-supervised approach as Self-Supervised Detection (\textbf{SSD}). 

This work can also be an opportunity to push for the following goals too:
\begin{itemize}
    \item \textit{How to validate detector performance on in-distribution data?} When claiming our detector have high TPR (validate all in-distribution images), we only test on the given training set. Should we be testing on a much larger rigorous set of images to claim that our detector does really have high TPR on the whole distribution, no just on the training set. Otherwise, the claims in the community are just getting overfitted to the images in our dataset, such as CIFAR10, which may not generalize to the whole distribution. Its similar to our ICCV idea of using transformations to expand in-distribution. 
    \item \textit{Using datasets representative of real-world setting?} What if we think of OOD detection from outlier/anomaly detection. Assuming that our only starting points is a set of inputs, where we don't even know which points are in or out distribution. We need to rethink the assumption that we always have a set of in-distribution images, as often we only have a set of in-distribution images, with OOD images present as label noise. Even more critical in learning without labels as the dataset are going to be even more uncontrolled.
    \item \textit{Asserting robust OOD detection.} In our earlier works we found that discriminative OOD detectors performs miserably when combined with robust training. \textbf{Would SSD better integrate with robust training}? But how do we craft an adversarial attacks and later design robust SSD.   
\end{itemize}

Note that our approach can also be integrated with supervised training, since supervised training achieves much better clustering in feature space, thus better detection performance than self-supervised features in out framework. 

\textbf{Assumptions.} Given the formulation of our approach, it will need calibration with some OOD data. We can provide results with two setting: 1) When no OOD data is available and we calibrate with random noise 2) When calibrating with OOD data. 


% Self-supervised learning is very effective in learning good clusters. However most methods operate under the assumption that fine-grained labels are available, thus supervised training. However, in real-world, OOD detection often translates to anomaly/outlier detection, where it may not be feasible to obtain labels in first place. Kind of like DeepSVM. Our question is how can be leverage the ability of these networks to do such amazing clustering to do better outlier detection. 

% We can then ask, how to develop robust self-supervised techniques focused on bringing robust clustering, thus better OOD detection performance in presence of adversary. Kind of giving more attention to our line of work. 

% I can also integrate it with my idea of using input transformation to help OOD detection.

==> old_sections/method.tex <==
Given a training set $\sX$ sample from $\pin$ consisting of training images $(\evx_1, \evx_2, \ldots, \evx_n)$, out objective to differentiate between $\sX$ and $\vz$, where $\vz \in \pood$. We first train a network with self-supervised method (SimCLR) to learn feature representations  $\sF = (\evf_1, \evf_2, \ldots, \evf_n)$. Our approach to develop a OOD detector on top of these representations takes the following steps:

\noindent \textbf{Step-1: Clustering.} In this step, we cluster the in-distribution features in $K$ clusters. Note that the choice of $K$ is pretty importance to success of out approach. We will use K-mean clustering in our work. It will return a set of centroids $\sC = (\evc_1, \evc_2, \ldots, \evc_k)$ for each clusters. Based on the distance to the cluster, the each point will be clustered with its nearest centroid, giving us a pseudo labels $\sY = (\evy_1, \evy_2, \ldots, \evy_n)$ for each training data point. 

\noindent \textbf{Step-2: Cluster-conditioned modelling of features vectors.} Our strategy is to develop a model of each cluster and use to detect OOD distribution data. The simplest model of all would be to use distance from cluster centroids. It includes, 1) Assign OOD features $\vf_z$ to the closest cluster $\evy_z$ 2) For each in-distribution data point in cluster $\evy_z$, find the distance from centroid, $S = \{d(\vf_i, \evc_{\evy_z}) | 1 \leq i \leq N, \evy_i = \evy_z\}$. Now $\vz$ will be OOD if $d(\vf_z, \evc_{\evy_z})\geq \delta$, where $\delta$ is determined from $\sS$ based on the pre-decided TPR (generally 95\%). 


\begin{figure}
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{temp/distance_low_entropy.png}
         \caption{Cluster where most examples are closest to the centroid (Tightest).}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{temp/distance_high_entropy.png}
         \caption{Cluster where most examples are farthest to the centroid (Loosest).}
     \end{subfigure}
    
    \caption{Two extremes of the clusters, tightest and loosest, obtained with Self-supervised training. Here we plot the distance distribution, for both in-distribution and OOD images belonging to each cluster. Again train data is used here as in-distribution.}
    \label{fig: distCluster}
\end{figure}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{temp/low_entropy_distribution.png}
         \caption{Cluster where most examples are closest to the centroid (Tightest).}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{temp/high_entropy_distribution.png}
         \caption{Cluster where most examples are farthest to the centroid (Loosest).}
     \end{subfigure}
    
    \caption{Simultaneously using distance from all clusters provide a better ability to differentiate between in and OOD data. Again train data is used here as in-distribution.}
\end{figure}


We show the results obtained with this approach in Figure~\ref{fig: distCluster}. It shows that distance from single cluster centroid will achieve poor OOD detection performance, since OOD data will be even closer to centroid in some clusters. 


We argue that dealing with each cluster individually is not the best strategy. We find that we should account distances from all clusters to better detect OOD data.\marginpar{\color{blue}\footnotesize Major-insight}. We first construct a vector $\vs$ where $\evs_{i} = -d(f, c_k)$ and $d$ is the $\normltwo$ distance. Our final score will be $H(\softmax(\vs))$, which is the entropy of the distribution obtained from distances from each cluster. We transform soft-max probabilities for simplicity. For better performance, we can also use distance like, Wasserstein, Mahalanobis distance to better compare with intra-cluster and inter-cluster data points. 


Hyper-parameters: Number of clusters (N), Temperature for softmax. 

==> old_sections/rel_work.tex <==
Note that we differ form the line of work which use self-supervision along with supervised training to improve OOD detectors~\cite{Winkens2020ContrastiveOOD, hendrycks2019SSLOOD}. We intend to use only Self-supervised learning, thus no labels, a setup which currently performs works in OOD detection. 

==> old_sections/results.tex <==
\begin{table}[!htb]
\centering
\caption{Comparison of our approach with state of the art detectors. Note that we are still using a sub-optimal setup (ResNet18 network, no hyperparameter tuning etc), as the goal was to get some quick numbers. Our method's performance is expected to improve further as we dig deeper. Note that all of these required labelled training data, and some even need OOD data for calibration, or pre-training on ImageNet. Our approach have none of these requirements and only require a set of unlabelled in-distribution images. We already achieve state-of-the-art FPR on CIFAR-10. Also CIFAR100 as OOD is hardest to detect, signalling that out methods performs best when the detection is hardest, a crucial innovation in OOD detection. We use features standardization following normalization, but removing former doesn't change much. Using best of distance or entropy$\times$distance, though entropy hurts with SVHN dataset and only helps barely when it does.}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{ccc|cc|cc}
\toprule
 & \multicolumn{2}{c}{CIFAR100} & \multicolumn{2}{c}{SVHN} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Gaussian \\ Noise\end{tabular}} \\  \cmidrule{2-3} \cmidrule{4-5} \cmidrule{6-7}
 & FPR (TPR=95)     & AUROC     & FPR (TPR=95)   & AUROC   & FPR (TPR=95)                              & AUROC  \\ \midrule
Softmax probability~\citep{hendrycks2016baseline} & -    & 86.4 & -   & 89.9 & -   & -     \\
ODIN~\cite{liang2017odin}          & -    & 85.8 & -   & 96.7 & -   & -     \\
Mahalanobis distance~\citep{lee2018unifiedOOD}    & -    & 88.2 & -   & 99.1 & -   & -     \\
Residual flows~\citep{zisselman2020resflow} & -    & 89.4 & -   & 99.1 & -   & -     \\
\textbf{Ours (100 clusters)}  & 57.1 & 87.5 & 13.0 & 97.6 & 2.4 & 98.9  \\
\textbf{Ours (500 clusters)}  & 57.3 & 87.9 & 12.1 & 97.8 & 2.3 & 98.7  \\
\textbf{Ours (2000 clusters)}  & \textbf{57.5} & \textbf{88.4} & \textbf{12.6} & \textbf{97.8} & 2.4 & 98.6  \\
%\textbf{Ours (10 clusters) + with labels}  & 64.6 & 84.3 & 46.3 & 91.8 & 3.1 & 99.1  \\
%\textbf{Ours (100 clusters) + with labels}  & 59.1 & 76.5 & 39.9 & 87.1 &  &   \\
%\textbf{Ours (500 clusters) + with labels}  & 58.3 & 77.2 & 38.6 & 88.3 &  &  \\  
Sup + Rotation-SSL~\citep{hendrycks2019SSLOOD} & -    & 90.9 & -   & 98.9 & -   & -     \\
Sup + SimCLR-SSL~\citep{Winkens2020ContrastiveOOD} (SOTA)  & \textbf{39.9} & \textbf{92.9} & \textbf{2.8} & \textbf{99.5} & 0.3 & 100.0 \\\bottomrule
\end{tabular}}
\end{table}


\begin{table}[!htb]
\centering
\caption{Using CIFAR100 as in-distribution, with ResNet18 network.}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{ccc|cc|cc}
\toprule
 & \multicolumn{2}{c}{CIFAR100} & \multicolumn{2}{c}{SVHN} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Gaussian \\ Noise\end{tabular}} \\  \cmidrule{2-3} \cmidrule{4-5} \cmidrule{6-7}
 & FPR (TPR=95)     & AUROC     & FPR (TPR=95)   & AUROC   & FPR (TPR=95)                              & AUROC  \\ \midrule
\textbf{Ours (100 clusters)}  & 73.4 & 78.8 & 26.9 & 91.7 & 4.4 & 98.7  \\
\textbf{Ours (500 clusters)}  & \textbf{68.6} & \textbf{80.8} & \textbf{20.2} & 93.1 & 3.0 & 98.8 \\
Sup + SimCLR-SSL~\citep{Winkens2020ContrastiveOOD} (SOTA)  &  81.8 & 78.3 & 23.3 & \textbf{95.6} & \textbf{0.2} & \textbf{99.9} \\ \bottomrule
\end{tabular}}
\end{table}


When labels are available, I find distance to closest cluster much better at OOD detection. With cifar10/cifar100 (in/ood) and 10 clusters combination it gets 46, 93.8 fpr and auroc respectively. With 100 clusters, we obtain 34 and 95.2 resectively. Increasingly number of clusters help but only with closest cluster distance, it hurts with entropy. \textit{If nothing else, just using cluster-conditional approach is sufficient to boost SOTA when labels are available.}


\subsection{Failure of statistical Outlier detection methods} Statistical methods for outlier detection assume that in-distribution data is generated from a certain distribution and OOD data will lie in its low-density regions. Generally, we assume that the distribution is Gaussian, where Mahalanobis distance can be used to characterize the equivalent high/low density regions. This works really well when we work with supervised training, since using Mahalanobis distance always works better than Euclidean, thus validating the assumption that Gaussian distribution is a nice prior. 

However, when working with OOD data (cifar10 as in-distribution) we observe that euclidean distance often works better than Mahalanobis, showing that Gaussian prior on data hurts more than it helps. Even more, performance with Mahalanobis distance gets even worse when we increase number of cluster, showing the individual clusters deviate even more from the Gaussian prior. Same behaviours occurs when we use a SupContrast model, i.e., model trained with both Supervised and Contrastive learning. Additionally, we find the SupContrast model, even with a single cluster, achieves SOTA on SVHN outlier dataset. This indicates that with labels, integrating them with Supervised learning might be more beneficial. 

\subsection{Beyond training dataset: validating TPR on training distribution}

As motivated earlier, it is imperative to validate the TPR of each detector on in-distribution images, going beyond the training set. With our detector, it is even more crucial, since a naive solution is assign each image a unique cluster. 
Don't forget to mention that performance on test can can certainly be used to check it.
\begin{table}[]
    \centering
    \caption{We select a select of 50k images from Tinyimages dataset which belongs to same class as CIFAR10, very likely in-distribution. When our detector is tuned to have TPR=95\% on CIFAR10 images, we test the TPR obtained in these tinyimages subset. Ideally, we would expect TPR=95\% on all indistribution images.}
    \begin{tabular}{ccc}
        \toprule
        Number of cluster &  TPR\\ \midrule
        100 &  87.9 \\
        500  & 82.3 \\
        2000 & 77.9 \\ \bottomrule
    \end{tabular}
\end{table}

List of our key observations is following:
\begin{itemize}
    \item We perform better in hard OOD setting than previous work. 
    \item Even with equal number of clusters, we beat previous SOTA on earlier datases. 
    \item 
\end{itemize}

==> sections/setup.tex <==





% \noindent \textbf{Architectures.} Given the large batch requirement of SimCLR, we use a ResNet50 network. Unlike previous works we don't use a highly over-parameterized wrn-28-10. 

% \noindent \textbf{Metrics.} Mention only a few and push the rest, both their definition and results, in appendix.

% \noindent \textbf{Datasets.} For each dataset mention which data points we consider as OOD and which as in-distribution.

% \subsubsection{Evaluation protocols}
% \noindent \textbf{Dataset based.} Here we use another dataset as OOD. Easiest to detect.

% \noindent \textbf{Class/Semantics based.} Here we use another dataset as OOD.

\noindent \textbf{Baselines.} We compare with earlier work on unsupervised modelling of in-distribution data. In particular, we use auto-encoders and autoregressive models as the baseline. We also compare with an equivalent supervised network along with with  existing state of the art.





